Reevaluation of Large Neighborhood Search for MAPF: Findings and Opportunities

Multi-Agent Path Finding (MAPF) aims to arrange collision-free goal-reaching paths for a group of agents. Anytime MAPF solvers based on large neighborhood search (LNS) have gained prominence recently due to their flexibility and scalability, leading to a surge of methods, especially those leveraging machine learning, to enhance neighborhood selection. However, several pitfalls exist and hinder a comprehensive evaluation of these new methods, which mainly include: 1) Lower than actual or incorrect baseline performance; 2) Lack of a unified evaluation setting and criterion; 3) Lack of a codebase or executable model for supervised learning methods. To address these challenges, we introduce a unified evaluation framework, implement prior methods, and conduct an extensive comparison of prominent methods. Our evaluation reveals that rule-based heuristics serve as strong baselines, while current learning-based methods show no clear advantage on time efficiency or improvement capacity. Our extensive analysis also opens up new research opportunities for improving MAPF-LNS, such as targeting high-delayed agents, applying contextual algorithms, optimizing replan order and neighborhood size, where machine learning can potentially be integrated. Code and data are available at https://github.com/ChristinaTan0704/mapf-lns-unified.

==> sup_table/bandit-ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

% \begin{table}[h]
%     \centering
%     \caption{'Uni-Bandit' represents our modified version of Bandit, where its second arm randomly selects a neighborhood size from {2, 4, 8, 16, 32} at each iteration. The performance of Uni-Bandit and Bandit is very close. This suggests that a better strategy for choosing neighborhood size could lead to improvements.}
%     \label{table:bandit-abliation}
%     \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}|cc|cc|cc|cc|cc|cc|@{}}
% \toprule
%                                                  &     & \multicolumn{2}{c|}{Delay} & \multicolumn{2}{c|}{AUC} &                                               &     & \multicolumn{2}{c|}{Delay} & \multicolumn{2}{c|}{AUC} \\ \midrule
% \multicolumn{1}{|c|}{map}                        & n   & Bandit     & Uni-Bandit    & Bandit    & Uni-Bandit   & \multicolumn{1}{c|}{map}                      & n   & Bandit     & Uni-Bandit    & Bandit    & Uni-Bandit   \\ \midrule
% \multicolumn{1}{|c|}{\multirow{5}{*}{empty}}     & 300 & 386.3      & 391.7         & 13.3      & 13.6         & \multicolumn{1}{c|}{\multirow{5}{*}{random}}  & 150 & 330.1      & 330.5         & 10.3      & 10.3         \\
% \multicolumn{1}{|c|}{}                           & 350 & 811.5      & 812.4         & 28.5      & 28.5         & \multicolumn{1}{c|}{}                         & 200 & 779.1      & 778.7         & 24.9      & 24.8         \\
% \multicolumn{1}{|c|}{}                           & 400 & 1537.2     & 1547.1        & 54.2      & 54.7         & \multicolumn{1}{c|}{}                         & 250 & 1507.3     & 1525.7        & 49.3      & 49.7         \\
% \multicolumn{1}{|c|}{}                           & 450 & 2753.7     & 2761.2        & 96.5      & 96.0         & \multicolumn{1}{c|}{}                         & 300 & 2746.0     & 2760.5        & 92.0      & 92.0         \\
% \multicolumn{1}{|c|}{}                           & 500 & 4318.5     & 4302.1        & 150.8     & 149.5        & \multicolumn{1}{c|}{}                         & 350 & 4564.1     & 4565.1        & 155.9     & 155.1        \\ \midrule
% \multicolumn{1}{|c|}{\multirow{5}{*}{warehouse}} & 150 & 107.9      & 111.8         & 3.6       & 3.7          & \multicolumn{1}{c|}{\multirow{5}{*}{ost003d}} & 200 & 158.2      & 163.8         & 8.3       & 8.3          \\
% \multicolumn{1}{|c|}{}                           & 200 & 239.4      & 234.3         & 8.0       & 7.9          & \multicolumn{1}{c|}{}                         & 300 & 532.8      & 484.3         & 33.4      & 31.2         \\
% \multicolumn{1}{|c|}{}                           & 250 & 414.2      & 414.0         & 14.2      & 14.5         & \multicolumn{1}{c|}{}                         & 400 & 1276.3     & 1327.3        & 75.2      & 75.0         \\
% \multicolumn{1}{|c|}{}                           & 300 & 669.5      & 677.2         & 23.8      & 24.1         & \multicolumn{1}{c|}{}                         & 500 & 3059.8     & 2873.5        & 163.6     & 155.8        \\
% \multicolumn{1}{|c|}{}                           & 350 & 1047.7     & 1042.6        & 38.2      & 39.1         & \multicolumn{1}{c|}{}                         & 600 & 6093.7     & 6430.8        & 311.4     & 321.9        \\ \midrule
% \multicolumn{1}{|c|}{\multirow{5}{*}{den520d}}   & 500 & 607.8      & 593.6         & 47.8      & 47.3         & \multicolumn{1}{c|}{\multirow{5}{*}{Paris}}   & 350 & 71.9       & 74.0          & 4.6       & 5.0          \\
% \multicolumn{1}{|c|}{}                           & 600 & 1247.0     & 1234.2        & 89.2      & 87.9         & \multicolumn{1}{c|}{}                         & 450 & 130.8      & 120.8         & 11.0      & 10.1         \\
% \multicolumn{1}{|c|}{}                           & 700 & 2297.4     & 2195.9        & 150.2     & 144.2        & \multicolumn{1}{c|}{}                         & 550 & 205.3      & 212.5         & 20.7      & 21.4         \\
% \multicolumn{1}{|c|}{}                           & 800 & 3330.3     & 3607.8        & 209.4     & 221.5        & \multicolumn{1}{c|}{}                         & 650 & 307.5      & 303.0         & 37.0      & 36.9         \\
% \multicolumn{1}{|c|}{}                           & 900 & 5343.5     & 5421.0        & 308.9     & 310.6        & \multicolumn{1}{c|}{}                         & 750 & 577.0      & 523.6         & 70.6      & 66.2         \\ \bottomrule
% \end{tabular}
% }
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

% \begin{table}[h]
%     \centering
%     \caption{\todo{update caption and value}}
%     \label{table:nns-svm-gen}
%     \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}|cc|cc|cc|cc|cc|cc|@{}}
% \toprule
%                                                  &     & \multicolumn{2}{c|}{Delay} & \multicolumn{2}{c|}{AUC} &                                               &     & \multicolumn{2}{c|}{Delay} & \multicolumn{2}{c|}{AUC} \\ \midrule
% \multicolumn{1}{|c|}{map}                        & n   & Bandit     & Uni-Bandit    & Bandit    & Uni-Bandit   & \multicolumn{1}{c|}{map}                      & n   & Bandit     & Uni-Bandit    & Bandit    & Uni-Bandit   \\ \midrule
% \multicolumn{1}{|c|}{\multirow{5}{*}{empty}}     & 300 & \textcolor{Red}{386.3}      & \textcolor{cyan}{391.7}         & \textcolor{Red}{13.3}      & \textcolor{cyan}{13.6}         & \multicolumn{1}{c|}{\multirow{5}{*}{random}}  & 150 & \textcolor{Red}{330.1}      & \textcolor{cyan}{330.5}         & \textcolor{cyan}{10.3}      & \textcolor{Red}{10.3}         \\
% \multicolumn{1}{|c|}{}                           & 350 & \textcolor{Red}{811.5}      & \textcolor{cyan}{812.4}         & \textcolor{Red}{28.5}      & \textcolor{cyan}{28.5}         & \multicolumn{1}{c|}{}                         & 200 & \textcolor{cyan}{779.1}      & \textcolor{Red}{778.7}         & \textcolor{cyan}{24.9}      & \textcolor{Red}{24.8}         \\
% \multicolumn{1}{|c|}{}                           & 400 & \textcolor{Red}{1537.2}     & \textcolor{cyan}{1547.1}        & \textcolor{Red}{54.2}      & \textcolor{cyan}{54.7}         & \multicolumn{1}{c|}{}                         & 250 & \textcolor{Red}{1507.3}     & \textcolor{cyan}{1525.7}        & \textcolor{Red}{49.3}      & \textcolor{cyan}{49.7}         \\
% \multicolumn{1}{|c|}{}                           & 450 & \textcolor{Red}{2753.7}     & \textcolor{cyan}{2761.2}        & \textcolor{cyan}{96.5}      & \textcolor{Red}{96.0}         & \multicolumn{1}{c|}{}                         & 300 & \textcolor{Red}{2746.0}     & \textcolor{cyan}{2760.5}        & \textcolor{Red}{92.0}      & \textcolor{cyan}{92.0}         \\
% \multicolumn{1}{|c|}{}                           & 500 & \textcolor{cyan}{4318.5}     & \textcolor{Red}{4302.1}        & \textcolor{cyan}{150.8}     & \textcolor{Red}{149.5}        & \multicolumn{1}{c|}{}                         & 350 & \textcolor{Red}{4564.1}     & \textcolor{cyan}{4565.1}        & \textcolor{Red}{155.9}     & \textcolor{cyan}{155.1}        \\ \midrule
% \multicolumn{1}{|c|}{\multirow{5}{*}{warehouse}} & 150 & \textcolor{Red}{107.9}      & \textcolor{cyan}{111.8}         & \textcolor{Red}{3.6}       & \textcolor{cyan}{3.7}          & \multicolumn{1}{c|}{\multirow{5}{*}{ost003d}} & 200 & \textcolor{Red}{158.2}      & \textcolor{cyan}{163.8}         & \textcolor{cyan}{8.3}       & \textcolor{Red}{8.3}          \\
% \multicolumn{1}{|c|}{}                           & 200 & \textcolor{cyan}{239.4}      & \textcolor{Red}{234.3}         & \textcolor{cyan}{8.0}       & \textcolor{Red}{7.9}          & \multicolumn{1}{c|}{}                         & 300 & \textcolor{cyan}{532.8}      & \textcolor{Red}{484.3}         & \textcolor{cyan}{33.4}      & \textcolor{Red}{31.2}         \\
% \multicolumn{1}{|c|}{}                           & 250 & \textcolor{cyan}{414.2}      & \textcolor{Red}{414.0}         & \textcolor{Red}{14.2}      & \textcolor{cyan}{14.5}         & \multicolumn{1}{c|}{}                         & 400 & \textcolor{Red}{1276.3}     & \textcolor{cyan}{1327.3}        & \textcolor{cyan}{75.2}      & \textcolor{Red}{75.0}         \\
% \multicolumn{1}{|c|}{}                           & 300 & \textcolor{Red}{669.5}      & \textcolor{cyan}{677.2}         & \textcolor{Red}{23.8}      & \textcolor{cyan}{24.1}         & \multicolumn{1}{c|}{}                         & 500 & \textcolor{cyan}{3059.8}     & \textcolor{Red}{2873.5}        & \textcolor{cyan}{163.6}     & \textcolor{Red}{155.8}        \\
% \multicolumn{1}{|c|}{}                           & 350 & \textcolor{cyan}{1047.7}     & \textcolor{Red}{1042.6}        & \textcolor{cyan}{38.2}      & \textcolor{Red}{39.1}         & \multicolumn{1}{c|}{}                         & 600 & \textcolor{Red}{6093.7}     & \textcolor{cyan}{6430.8}        & \textcolor{Red}{311.4}     & \textcolor{cyan}{321.9}        \\ \midrule
% \multicolumn{1}{|c|}{\multirow{5}{*}{den520d}}   & 500 & \textcolor{cyan}{607.8}      & \textcolor{Red}{593.6}         & \textcolor{cyan}{47.8}      & \textcolor{Red}{47.3}         & \multicolumn{1}{c|}{\multirow{5}{*}{Paris}}   & 350 & \textcolor{Red}{71.9}       & \textcolor{cyan}{74.0}          & \textcolor{Red}{4.6}       & \textcolor{cyan}{5.0}          \\
% \multicolumn{1}{|c|}{}                           & 600 & \textcolor{cyan}{1247.0}     & \textcolor{Red}{1234.2}        & \textcolor{cyan}{89.2}      & \textcolor{Red}{87.9}         & \multicolumn{1}{c|}{}                         & 450 & \textcolor{cyan}{130.8}      & \textcolor{Red}{120.8}         & \textcolor{cyan}{11.0}      & \textcolor{Red}{10.1}         \\
% \multicolumn{1}{|c|}{}                           & 700 & \textcolor{cyan}{2297.4}     & \textcolor{Red}{2195.9}        & \textcolor{cyan}{150.2}     & \textcolor{Red}{144.2}        & \multicolumn{1}{c|}{}                         & 550 & \textcolor{Red}{205.3}      & \textcolor{cyan}{212.5}         & \textcolor{Red}{20.7}      & \textcolor{cyan}{21.4}         \\
% \multicolumn{1}{|c|}{}                           & 800 & \textcolor{Red}{3330.3}     & \textcolor{cyan}{3607.8}        & \textcolor{Red}{209.4}     & \textcolor{cyan}{221.5}        & \multicolumn{1}{c|}{}                         & 650 & \textcolor{cyan}{307.5}      & \textcolor{Red}{303.0}         & \textcolor{cyan}{37.0}      & \textcolor{Red}{36.9}         \\
% \multicolumn{1}{|c|}{}                           & 900 & \textcolor{Red}{5343.5}     & \textcolor{cyan}{5421.0}        & \textcolor{Red}{308.9}     & \textcolor{cyan}{310.6}        & \multicolumn{1}{c|}{}                         & 750 & \textcolor{cyan}{577.0}      & \textcolor{Red}{523.6}         & \textcolor{cyan}{70.6}      & \textcolor{Red}{66.2}         \\ \bottomrule
% \end{tabular}
% }
% \end{table}



\begin{table}[h]
    \centering
    \caption{'Uni-Bandit' represents our modified version of Bandit, where it randomly selects a neighborhood size from ${2, 4, 8, 16, 32}$ at each iteration instead of using the neighbourhood selection arm. The better results are marked in bold. The performance of Uni-Bandit and Bandit is very close. This suggests that a better strategy for choosing neighborhood size could lead to improvements.}
    \label{table:bandit-abliation}
    \resizebox{\textwidth}{!}{
\begin{tabular}{@{}|cc|cc|cc|cc|cc|cc|@{}}
\toprule
                                                 &     & \multicolumn{2}{c|}{Delay} & \multicolumn{2}{c|}{AUC} &                                               &     & \multicolumn{2}{c|}{Delay} & \multicolumn{2}{c|}{AUC} \\ \midrule
\multicolumn{1}{|c|}{map}                        & n   & Bandit     & Uni-Bandit    & Bandit    & Uni-Bandit   & \multicolumn{1}{c|}{map}                      & n   & Bandit     & Uni-Bandit    & Bandit    & Uni-Bandit   \\ \midrule
\multicolumn{1}{|c|}{\multirow{5}{*}{empty}}     & 300 & \textbf{386.3}      & \textcolor{black}{391.7}         & \textbf{13.3}      & \textcolor{black}{13.6}         & \multicolumn{1}{c|}{\multirow{5}{*}{random}}  & 150 & \textbf{330.1}      & \textcolor{black}{330.5}         & \textcolor{black}{10.3}      & \textbf{10.3}         \\
\multicolumn{1}{|c|}{}                           & 350 & \textbf{811.5}      & \textcolor{black}{812.4}         & \textbf{28.5}      & \textcolor{black}{28.5}         & \multicolumn{1}{c|}{}                         & 200 & \textcolor{black}{779.1}      & \textbf{778.7}         & \textcolor{black}{24.9}      & \textbf{24.8}         \\
\multicolumn{1}{|c|}{}                           & 400 & \textbf{1537.2}     & \textcolor{black}{1547.1}        & \textbf{54.2}      & \textcolor{black}{54.7}         & \multicolumn{1}{c|}{}                         & 250 & \textbf{1507.3}     & \textcolor{black}{1525.7}        & \textbf{49.3}      & \textcolor{black}{49.7}         \\
\multicolumn{1}{|c|}{}                           & 450 & \textbf{2753.7}     & \textcolor{black}{2761.2}        & \textcolor{black}{96.5}      & \textbf{96.0}         & \multicolumn{1}{c|}{}                         & 300 & \textbf{2746.0}     & \textcolor{black}{2760.5}        & \textbf{92.0}      & \textcolor{black}{92.0}         \\
\multicolumn{1}{|c|}{}                           & 500 & \textcolor{black}{4318.5}     & \textbf{4302.1}        & \textcolor{black}{150.8}     & \textbf{149.5}        & \multicolumn{1}{c|}{}                         & 350 & \textbf{4564.1}     & \textcolor{black}{4565.1}        & \textbf{155.9}     & \textcolor{black}{155.1}        \\ \midrule
\multicolumn{1}{|c|}{\multirow{5}{*}{warehouse}} & 150 & \textbf{107.9}      & \textcolor{black}{111.8}         & \textbf{3.6}       & \textcolor{black}{3.7}          & \multicolumn{1}{c|}{\multirow{5}{*}{ost003d}} & 200 & \textbf{158.2}      & \textcolor{black}{163.8}         & \textcolor{black}{8.3}       & \textbf{8.3}          \\
\multicolumn{1}{|c|}{}                           & 200 & \textcolor{black}{239.4}      & \textbf{234.3}         & \textcolor{black}{8.0}       & \textbf{7.9}          & \multicolumn{1}{c|}{}                         & 300 & \textcolor{black}{532.8}      & \textbf{484.3}         & \textcolor{black}{33.4}      & \textbf{31.2}         \\
\multicolumn{1}{|c|}{}                           & 250 & \textcolor{black}{414.2}      & \textbf{414.0}         & \textbf{14.2}      & \textcolor{black}{14.5}         & \multicolumn{1}{c|}{}                         & 400 & \textbf{1276.3}     & \textcolor{black}{1327.3}        & \textcolor{black}{75.2}      & \textbf{75.0}         \\
\multicolumn{1}{|c|}{}                           & 300 & \textbf{669.5}      & \textcolor{black}{677.2}         & \textbf{23.8}      & \textcolor{black}{24.1}         & \multicolumn{1}{c|}{}                         & 500 & \textcolor{black}{3059.8}     & \textbf{2873.5}        & \textcolor{black}{163.6}     & \textbf{155.8}        \\
\multicolumn{1}{|c|}{}                           & 350 & \textcolor{black}{1047.7}     & \textbf{1042.6}        & \textcolor{black}{38.2}      & \textbf{39.1}         & \multicolumn{1}{c|}{}                         & 600 & \textbf{6093.7}     & \textcolor{black}{6430.8}        & \textbf{311.4}     & \textcolor{black}{321.9}        \\ \midrule
\multicolumn{1}{|c|}{\multirow{5}{*}{den520d}}   & 500 & \textcolor{black}{607.8}      & \textbf{593.6}         & \textcolor{black}{47.8}      & \textbf{47.3}         & \multicolumn{1}{c|}{\multirow{5}{*}{Paris}}   & 350 & \textbf{71.9}       & \textcolor{black}{74.0}          & \textbf{4.6}       & \textcolor{black}{5.0}          \\
\multicolumn{1}{|c|}{}                           & 600 & \textcolor{black}{1247.0}     & \textbf{1234.2}        & \textcolor{black}{89.2}      & \textbf{87.9}         & \multicolumn{1}{c|}{}                         & 450 & \textcolor{black}{130.8}      & \textbf{120.8}         & \textcolor{black}{11.0}      & \textbf{10.1}         \\
\multicolumn{1}{|c|}{}                           & 700 & \textcolor{black}{2297.4}     & \textbf{2195.9}        & \textcolor{black}{150.2}     & \textbf{144.2}        & \multicolumn{1}{c|}{}                         & 550 & \textbf{205.3}      & \textcolor{black}{212.5}         & \textbf{20.7}      & \textcolor{black}{21.4}         \\
\multicolumn{1}{|c|}{}                           & 800 & \textbf{3330.3}     & \textcolor{black}{3607.8}        & \textbf{209.4}     & \textcolor{black}{221.5}        & \multicolumn{1}{c|}{}                         & 650 & \textcolor{black}{307.5}      & \textbf{303.0}         & \textcolor{black}{37.0}      & \textbf{36.9}         \\
\multicolumn{1}{|c|}{}                           & 900 & \textbf{5343.5}     & \textcolor{black}{5421.0}        & \textbf{308.9}     & \textcolor{black}{310.6}        & \multicolumn{1}{c|}{}                         & 750 & \textcolor{black}{577.0}      & \textbf{523.6}         & \textcolor{black}{70.6}      & \textbf{66.2}         \\ \bottomrule
\end{tabular}
}
\end{table}


==> sup_table/eecbs_main_result.tex <==
\begin{table}[h!]
\caption{Final delays and AUC (divided by 10k) of different methods with best neighborhood size, evaluated on maps with medium number of agents within 300s and 60s. The agent numbers are shown after the name of a map. Initial solutions are provided by EECBS. Highlighted are the results ranked \textcolor{Red}{first}, and \textcolor{cyan}{second}.}
\label{table:mid-agent-eecbs-delay-auc}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccccccccccc}
\toprule
\multirow{3}{*}{\textbf{Methods}} & \multicolumn{12}{c}{\textbf{Init solution: EECBS, Time: 300s}}  \\
& \multicolumn{2}{c}{\textbf{empty}+400} & \multicolumn{2}{c}{\textbf{random}+250} & \multicolumn{2}{c}{\textbf{warehouse}+250} & \multicolumn{2}{c}{\textbf{ost003d}+400} & \multicolumn{2}{c}{\textbf{den520d}+700} & \multicolumn{2}{c}{\textbf{Paris}+550} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13}
& Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC\\
\midrule
RandomWalk & \textcolor{Red}{1116.1} & \textcolor{Red}{38.47} & - & - &  \textcolor{Red}{402.03} & \textcolor{cyan}{12.88} &-&-&-&-&-&-\\
Intersection & 1228.2 & 41.12 & - & - & 470.4 & 15.60 &-&-&-&-&-&-\\
Random & 1311.3 & 43.47 & - & - & 440.4 & 14.07 &-&-&-&-&-&-\\
Adaptive & \textcolor{cyan}{1170.1} & \textcolor{cyan}{39.03} & - & - & 408.8 & 13.14 &-&-&-&-&-&-\\
RandomWalkProb & 1202.1 & 39.86 & - & - & 430.5 & 14.16 &-&-&-&-&-&-\\
\midrule
Our-SVM & 1252.44 & 47.82 & - & - & 408.12 & 13.24 &-&-&-&-&-&-\\
Our-Neural & 1506.54 & 51.73 & - & - & 524.0 & 17.30 &-&-&-&-&-&-\\
Bandit & 1250.0 & 42.32 & - & - & \textcolor{cyan}{404.76} & \textcolor{Red}{12.69} &-&-&-&-&-&-\\
Orig-SVM & 1313.6 & 51.84 & - & - & 417.2 & 13.69 &-&-&-&-&-&-\\
Orig-Neural & 1409.7 & 53.51 & - & - & 497.1 & 18.30 &-&-&-&-&-&-\\
\midrule

& \multicolumn{12}{c}{\textbf{Init solution: LaCAM2, Time: 60s}}  \\
\midrule
RandomWalk & \textcolor{Red}{1313.84} & \textcolor{cyan}{9.42} & - & - &  \textcolor{cyan}{436.93} & \textcolor{cyan}{2.94} &-&-&-&-&-&-\\
Intersection & 1412.44 & 10.13 & - & - & 549.7 & 3.72 &-&-&-&-&-&-\\
Random & 1438.77 & 9.86 & - & - & 474.47 & 3.25 &-&-&-&-&-&-\\
Adaptive & \textcolor{cyan}{1342.73} & \textcolor{Red}{9.32} & - & - & 446.62 & 3.07 &-&-&-&-&-&-\\
RandomWalkProb & 1369.38 & 9.72 & - & - & 488.39 & 3.32 &-&-&-&-&-&-\\
\midrule
Our-SVM & 1826.71 & 14.57 & - & - & 450.96 & 3.13 &-&-&-&-&-&-\\
Our-Neural &  1823.47 & 13.10 & - & - & 599.86 & 4.07 &-&-&-&-&-&-\\
Bandit & 1473.95 & 10.60 & - & - & \textcolor{Red}{425.42} & \textcolor{Red}{2.81} &-&-&-&-&-&-\\
Orig-SVM & 1968.86 & 15.70 & - & - & 455.75 & 3.48 &-&-&-&-&-&-\\
Orig-Neural & 1946.74 & 15.82 & - & - & 694.49 & 4.74 &-&-&-&-&-&-\\
\bottomrule
\end{tabular}
}
\end{table}


==> sup_table/lacam2_main_result.tex <==

\begin{table}[h!]
\caption{Final delays and AUC (divided by 10k) of different methods with best neighborhood size, evaluated on maps with medium number of agents within 300s and 60s. The agent numbers are shown after the name of a map. Initial solutions are provided by LaCAM2. Highlighted are the results ranked \textcolor{Red}{first}, and \textcolor{cyan}{second}.}
\label{table:mid-agent-lacam2-delay-auc}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccccccccccc}
\toprule
\multirow{3}{*}{\textbf{Methods}} & \multicolumn{12}{c}{\textbf{Init solution: LaCAM2, Time: 300s}}  \\
% \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
& \multicolumn{2}{c}{\textbf{empty}+400} & \multicolumn{2}{c}{\textbf{random}+250} & \multicolumn{2}{c}{\textbf{warehouse}+250} & \multicolumn{2}{c}{\textbf{ost003d}+400} & \multicolumn{2}{c}{\textbf{den520d}+700} & \multicolumn{2}{c}{\textbf{Paris}+550} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13}
& Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC\\
\midrule
RandomWalk &  \textcolor{Red}{1447.93} & \textcolor{Red}{52.87} & \textcolor{cyan}{1472.74} & \textcolor{cyan}{50.15} & 430.02 & \textcolor{cyan}{18.10} & 430.02 & \textcolor{cyan}{18.10} & 933.10 & 86.97 & 198.04 & \textcolor{cyan}{10.72} \\
Intersection & 1593.40 & 58.25 & 1537.20 & 53.64 & 698.50 & 47.96 & 1849.61 & 97.46 & 3163.02 & 169.04 & 776.46 & 58.17 \\
Random & 1756.18 & 61.44 & 1613.49 & 54.29 & 562.40 & 29.80 & 1488.17 & 91.63 & 2782.67 & 176.17 & 466.87 & 48.55 \\
Adaptive & \textcolor{cyan}{1476.49} & \textcolor{cyan}{53.10} & 1506.69 & 50.95 & \textcolor{Red}{424.93} & 19.31 & 805.22 & 55.20 & 1075.19 & 91.26 & 194.79 & 15.25 \\
RandomWalkProb & 1484.35 & 53.88 & 1494.11 & 50.56 & 446.69 & 20.09 & \textcolor{Red}{622.85} & \textcolor{Red}{38.92} & \textcolor{Red}{622.43} & \textcolor{Red}{55.41} & \textcolor{Red}{183.27} & \textcolor{Red}{9.73} \\
\midrule
Our-SVM & 1692.37 & 83.42 & 1521.21 & 60.13 & 444.61 & 41.10 & 762.46 & 96.38 & \textcolor{cyan}{660.71}  & 138.12 & \textcolor{cyan}{184.72} & 33.00 \\
Our-Neural & 2094.76 & 81.62 & 1747.14 & 63.64 & 782.08 & 38.25 & \textcolor{cyan}{675.32} & \textcolor{cyan}{46.35} & 816.58 & \textcolor{cyan}{85.94} & 228.87 & 17.10 \\
Bandit & 1579.02 & 57.57 & \textcolor{Red}{1456.33} & \textcolor{Red}{48.61} & \textcolor{cyan}{426.15} & \textcolor{Red}{16.62} & 1253.27 & 78.42 & 2439.18 & 165.78 & 210.23 & 28.72 \\
Orig-SVM & 1857.49 & 97.55 & 1604.75 & 67.43 & 445.08 & 36.29 & 1083.73 & 123.70 & 2258.95 & 327.11 & 200.56 & 105.33 \\
Orig-Neural & 1614.31 & 74.40 & 1698.53 & 70.88 & 961.45 & 127.21 & 5277.44 & 310.16 & 15529.00 & 726.01 & 2643.73 & 261.44 \\
\midrule

& \multicolumn{12}{c}{\textbf{Init solution: LaCAM2, Time: 60s}}  \\
\midrule
RandomWalk & \textcolor{Red}{1845.71} & 15.22 & \textcolor{Red}{1698.27} & 13.15 & \textcolor{cyan}{470.07} & \textcolor{cyan}{7.20} & 1717.20 & 27.23 &  \textcolor{cyan}{2641.97} & \textcolor{cyan}{46.77} & \textcolor{cyan}{217.23} & \textcolor{cyan}{5.90} \\
Intersection & 2030.12 & 16.65 & 1830.54 & 14.51 & 1731.44 & 24.94 & 3618.77 & 41.14 & 6254.74 & 71.26 & 2269.39 & 27.09 \\
Random & 2130.49 & 16.44 & 1832.18 & 14.00 & 813.23 & 14.31 & 3750.10 & 41.21 & 7336.47 & 76.57 & 2110.06 & 27.09 \\
Adaptive & \textcolor{cyan}{1861.78} & \textcolor{Red}{14.81} & 1733.45 & \textcolor{cyan}{13.13} & 485.38 & 8.66 & 2023.81 & 29.13 & 3418.03 & 51.79 & 236.39 & 7.43 \\
RandomWalkProb & 1877.6 & \textcolor{cyan}{15.07} & 1711.63 & 13.14 & 537.08 & 8.84 & \textcolor{Red}{1143.82} & \textcolor{Red}{21.44} & \textcolor{Red}{1494.63} & \textcolor{Red}{36.19} & \textcolor{Red}{202.53} & \textcolor{Red}{5.20} \\
\midrule
Our-SVM &  3679.88 & 30.54 & 2274.59 & 19.86 & 1144.09 & 28.78 & 5073.09 & 52.66 & 6070.30 & 97.46 & 545.62 & 27.87 \\
Our-Neural &  2981.60 & 24.63 & 2246.29 & 18.19 & 1201.94 & 16.08 & \textcolor{cyan}{1541.18} & \textcolor{cyan}{25.71} & 2933.96 & 56.16 & 350.31 & 10.91 \\
Bandit & 2027.85 & 16.12 & \textcolor{Red}{1652.80} & \textcolor{Red}{12.23} & \textcolor{Red}{466.79} & \textcolor{Red}{6.09} & 3118.42 & 35.25 & 7198.20 & 75.06 & 960.80 & 20.78 \\
Orig-SVM & 4503.57 & 34.83 & 2587.10 & 23.63 & 872.97 & 24.43 & 6332.78 & 69.58 & 19781.82 & 158.77 & 7313.95 & 78.02 \\
Orig-Neural & 2942.81 & 27.94 & 2674.51 & 23.30 & 7424.49 & 60.45 & 14720.52 & 102.22 & 30196.75 & 191.74 & 13938.81 & 99.11 \\
\bottomrule
\end{tabular}
}
\end{table}



\begin{table}[h!]
\caption{Final delays and AUC (divided by 10k) of different methods with best neighborhood size, evaluated on maps with largest number of agents within 300s and 60s. The agent numbers are shown after the name of a map. Initial solutions are provided by LaCAM2. Highlighted are the results ranked \textcolor{Red}{first}, and \textcolor{cyan}{second}.}
\label{table:max-agent-lacam2-delay-auc}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccccccccccc}
\toprule
\multirow{3}{*}{\textbf{Methods}} & \multicolumn{12}{c}{\textbf{Init solution: LaCAM2, Time: 300s}}  \\
& \multicolumn{2}{c}{\textbf{empty}+500} & \multicolumn{2}{c}{\textbf{random}+350} & \multicolumn{2}{c}{\textbf{warehouse}+350} & \multicolumn{2}{c}{\textbf{ost003d}+600} & \multicolumn{2}{c}{\textbf{den520d}+900} & \multicolumn{2}{c}{\textbf{Paris}+750} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13}
& Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC & Delay & AUC \\
\midrule
RandomWalk &  \textcolor{Red}{4237.71} & \textcolor{Red}{155.66} & \textcolor{Red}{4341.57} & 169.08 & \textcolor{cyan}{1043.00} & \textcolor{cyan}{56.83} & 7513.99 & 450.57 & 2486.09 & 201.86 & 373.15 & 27.46 \\
Intersection &  4448.52 & 162.94 & 4622.23 & 184.56 & 2010.98 & 158.73 & 10394.78 & 529.43 & 6425.98 & 351.11 & 1821.18 & 123.22 \\
Random &  4828.23 & 171.83 & 4683.93 & 186.63 & 1509.02 & 92.99 & 12466.14 & 613.46 & 6923.52 & 396.91 & 1362.59 & 115.02 \\
Adaptive &  4374.48 & 156.47 & 4406.49 & \textcolor{Red}{163.77} & 1054.99 & 63.12 & 8216.92 & 469.61 & 2819.86 & 225.56 & 385.84 & \textcolor{cyan}{39.40} \\
RandomWalkProb & \textcolor{cyan}{4335.71} & 159.82 & \textcolor{cyan}{4367.54} & \textcolor{cyan}{166.60} & 1130.83 & 67.02 & \textcolor{Red}{5874.98}  & \textcolor{Red}{383.28} & \textcolor{Red}{1381.97} & \textcolor{Red}{151.59} & \textcolor{Red}{366.01} & \textcolor{Red}{23.87} \\
\midrule
Our-SVM &  5194.85 & 223.50 & 5162.68 & 241.24 & \textcolor{Red}{1042.40} & 100.43 & 13066.61 & 618.02 & \textcolor{cyan}{2058.55} & 335.36 & \textcolor{cyan}{369.93} & 108.04 \\
Our-Neural &  5808.02 & 221.09 & 5886.46 & 241.76 & 1907.01 & 101.40 & 8469.09 & 465.00 & 2067.14 & \textcolor{cyan}{217.58} & 498.84 & 47.80 \\
Bandit &  4772.62 & 173.84 & 4598.53 & 169.33 & \textcolor{cyan}{1067.58} & \textcolor{cyan}{49.67} & \textcolor{cyan}{7244.61} & \textcolor{cyan}{400.06} & 5595.39 & 346.67 & 627.28 & 87.12 \\
Orig-SVM &  5793.57 & 243.96 & 5983.60 & 262.86 & 1097.62 & 112.19 & 10153.89 & 625.01 & 15199.04 & 723.88 & 616.29 & 261.45 \\
Orig-Neural &  6085.27 & 242.91 & 7438.82 & 312.23 & 5255.12 & 361.57 & 25804.48 & 962.95 & 31693.98 & 1246.97 & 13831.51 & 656.43 \\
\midrule

& \multicolumn{12}{c}{\textbf{Init solution: LaCAM2, Time: 60s}}  \\
\midrule
RandomWalk & \textcolor{Red}{5605.03} & 43.83 & \textcolor{cyan}{5535.21} & 46.40 & \textcolor{red}{1421.02} & \textcolor{cyan}{30.36} & 20549.41 & 162.98 & \textcolor{cyan}{8274.09} & \textcolor{cyan}{108.85} & 1845.70 & 15.20 \\
Intersection & 5895.29 & 45.63 & 6027.22 & 50.65 & 7091.60 & 72.70 & 21652.95 & 171.51 & 13090.97 & 138.60 & 2030.10 & 16.60 \\
Random & 6075.96 & \textcolor{cyan}{43.22} & 5764.85 & 46.66 & 2764.39 & 49.76 & 22508.10 & 173.33 & 16636.17 & 154.71 & 2130.40 & 16.40 \\
Adaptive & \textcolor{cyan}{5631.04} & \textcolor{Red}{41.84} & 5544.01 & \textcolor{Red}{45.50} & 1577.07 & 33.52 & 20281.28 & 160.24 & 9786.31 & 114.84 & 1861.70 & \textcolor{cyan}{14.80} \\
RandomWalkProb & 5790.5 & 44.6 & \textcolor{Red}{5463.1} & \textcolor{cyan}{45.6} & \textcolor{cyan}{1514.3} & 34.2 & \textcolor{cyan}{17560.6} & \textcolor{cyan}{153.3} & \textcolor{Red}{4788.8} & \textcolor{Red}{86.8} & \textcolor{Red}{462.8} & \textcolor{Red}{13.5} \\
\midrule
Our-SVM &  8973.59 & 63.69 & 10463.71 & 75.41 & 4450.79 & 63.28 & 26121.51 & 188.01 & 18143.86 & 185.35 & 5088.31 & 85.13 \\
Our-Neural &  8475.42 & 60.29 & 9710.57 & 71.69 & 3366.54 & 44.95 & 20302.89 & 162.10 & 9199.73 & 126.87 & \textcolor{cyan}{1080.62} & 32.78 \\
Bandit & 6294.53 & 48.15 & 5943.98 & 49.94 & 1334.33 & \textcolor{Red}{22.40} & \textcolor{Red}{16993.81} & \textcolor{Red}{146.55} & 14398.93 & 144.19 & 3742.99 & 52.95 \\
Orig-SVM & 9866.16 & 67.50 & 10815.58 & 76.92 & 5331.10 & 71.10 & 29866.42 & 204.27 & 30208.88 & 191.02 & 18276.64 & 146.27 \\
Orig-Neural & 9953.82 & 68.31 & 12978.23 & 83.86 & 17479.58 & 119.62 & 36312.50 & 224.55 & 47864.21 & 297.39 & 27245.04 & 175.07 \\
\bottomrule

\end{tabular}
}
\end{table}
  


==> sup_table/nns_comp.tex <==

% \begin{table}[h]
% \caption{Delay elimination of trained Orig-Neural-LNS within 100 iterations and reported values by~\citet{yan2024neural},  if starting from a roughly equivalent point of delays. 'n' represent the number of agents in the map. \todo{update the table format: make our and reported under initial delays, start ***} }
%   \label{table:neural-100iter}
%   \centering
%   {\small
%   \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%         \multirow{2}{*}{Map} &  \multirow{2}{*}{n} & & Initial & Starting & Delay \\
%         & &  &delays & iteration & elimination  \\
%     \midrule
%     \multirow{2}{*}{empty} &  \multirow{2}{*}{300} & Our & 3140.7 & 0 & 2202\\
%     % \cline{3-6}
%     & & Reported & 3200 & 0 & 1850\\
%   \midrule
%   \multirow{2}{*}{warehouse} &  \multirow{2}{*}{100} & Our & 5731.8 & 2 & 4908\\
%   % \cline{3-6}
%   & & Reported & 5500& 0 & 4700\\ 
%   \midrule
%   \multirow{2}{*}{ost003d} &  \multirow{2}{*}{100} & Our & 8690.4 & 39 & 4585.1\\
%   & & Reported & 8600 & 0 & 5000\\
%   \midrule
%   \multirow{2}{*}{den520d} &  \multirow{2}{*}{200} & Our & 20510.2 & 19 & 12721.3\\
%   & & Reported & 20500 & 0 & 14500\\
%   \bottomrule
%   \end{tabular}
%   }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\caption{Delay elimination of trained Orig-Neural-LNS within 100 iterations and reported values by~\citet{yan2024neural},  if starting from a roughly equivalent point of delays. 'n' represent the number of agents in the map. }
\label{table:neural-100iter}
\centering
\begin{tabular}{@{}cc|cc|cc|cc@{}}
\toprule
                               &     & \multicolumn{2}{c|}{Initial delays} & \multicolumn{2}{c|}{Starting Iteration} & \multicolumn{2}{c}{Delay reduction} \\ \midrule
\multicolumn{1}{c|}{Map}       & n   & Our              & Reported         & Our              & Reported             & Our              & Reported         \\ \midrule
\multicolumn{1}{c|}{empty}     & 300 & 3140.7           & 3200             & 0                & 0                    & 2202             & 1850             \\
\multicolumn{1}{c|}{warehouse} & 100 & 5731.8           & 5500             & 2                & 0                    & 4908             & 4700             \\
\multicolumn{1}{c|}{ost003d}   & 100 & 8690.4           & 8600             & 39               & 0                    & 4585.1           & 5000             \\
\multicolumn{1}{c|}{den520d}   & 200 & 20510.2          & 20500            & 19               & 0                    & 12721.3          & 14500            \\ \bottomrule
\end{tabular}
\end{table}

==> sup_table/nns_svm_gen.tex <==



\begin{table}[h]
    \centering
    
    \caption{\textbf{Neighbourhood Size, Removal Strategy, Agent Number, Initial solver Generalization for Ours-SVM-LNS and Ours-Neural-LNS}. 'NB' represents the neighborhood size. RNWLK, ADP, and RNWLKPB stand for RandomWalk, Adaptive, and RandomWalkProb, respectively. Every two rows in a block represent a set of generalization experiments on one map; the top row shows generalized results, with the bottom row for comparison. We use 23 solved scenes on the random map and Paris to test the generalization ability of EECBS, as other scenes in random and den520d are unsolvable by EECBS within the time limit. Overall, there is no significant advantage to training the map on each different setting.} 
    \resizebox{\textwidth}{!}{
    \label{table:nns-svm-gen-nb-agent-sol-strategy}
    \begin{tabular}{@{}cccccccccccccc@{}}
    \toprule
    \multicolumn{7}{c|}{\textbf{Neighbourhood   Size Generalization}}                                                                                                                               & \multicolumn{7}{|c}{\textbf{Removal Strategy   Generalization}}                                                                                                              \\ \midrule
    \multicolumn{1}{c|}{}                         & \multicolumn{2}{c|}{NB}          & \multicolumn{2}{c|}{Our-SVM}          & \multicolumn{2}{c|}{Our-NNS}          & \multicolumn{1}{c|}{}                         & \multicolumn{2}{c|}{Removal Strategy}                  & \multicolumn{2}{c|}{Our-SVM}          & \multicolumn{2}{c}{Our-NNS} \\ \midrule
    \multicolumn{1}{c|}{Map}                      & \multicolumn{1}{c}{Train} & \multicolumn{1}{c|}{Infer} & Delay   & \multicolumn{1}{c|}{AUC}    & Delay   & \multicolumn{1}{c|}{AUC}    & \multicolumn{1}{c|}{Map}                      & Train          & \multicolumn{1}{c|}{Infer}    & Delay   & \multicolumn{1}{c|}{AUC}    & Delay         & AUC         \\ \midrule
    \multicolumn{1}{c|}{random}            & \multicolumn{1}{c|}{8}     & \multicolumn{1}{c|}{16}    & \textcolor{black}{1688.17} & \multicolumn{1}{c|}{61.32}  & \textcolor{black}{1829.46} & \multicolumn{1}{c|}{\textcolor{black}{61.94}}  & \multicolumn{1}{c|}{random}  &  \multicolumn{1}{c|}{RNWLK}    & \multicolumn{1}{c|}{ADP} & 1576.10 & \multicolumn{1}{c|}{56.64} & 1752.68       & 58.29       \\
    \multicolumn{1}{c|}{+250}                         & \multicolumn{1}{c|}{16}    & \multicolumn{1}{c|}{16}    & 1700.6  & \multicolumn{1}{c|}{\textcolor{black}{60.65}}  & 1912.3  & \multicolumn{1}{c|}{64.79}  & \multicolumn{1}{c|}{+250}                         &   \multicolumn{1}{c|}{ADP}      & \multicolumn{1}{c|}{ADP} & \textcolor{black}{1566.19} & \multicolumn{1}{c|}{\textcolor{black}{55.26}} & 1735.02       & 57.99       \\\midrule
    \multicolumn{1}{c|}{den520d}                 & \multicolumn{1}{c|}{16}    & \multicolumn{1}{c|}{8}     & \textcolor{black}{837.6}   & \multicolumn{1}{c|}{\textcolor{black}{97.82}}  & 1485.69 & \multicolumn{1}{c|}{76.82}  & \multicolumn{1}{c|}{den520d} & \multicolumn{1}{c|}{RNWLKPB}  & \multicolumn{1}{c|}{ADP} & 1792.96 & \multicolumn{1}{c|}{168.26} & 2759.75       & 126.89      \\
    \multicolumn{1}{c|}{+700}                         & \multicolumn{1}{c|}{8}     & \multicolumn{1}{c|}{8}     & 861.52  & \multicolumn{1}{c|}{98.48}  & \textcolor{black}{1150.04} & \multicolumn{1}{c|}{\textcolor{black}{62.37}}  & \multicolumn{1}{c|}{+700}                         &   \multicolumn{1}{c|}{ADP}     & \multicolumn{1}{c|}{ADP} & 1662.87 & \multicolumn{1}{c|}{164.28} & 1964.9        & 93.23       \\ \bottomrule
    \multicolumn{7}{c|}{\textbf{Agent Number Generalization}}                                                                                                                                    & \multicolumn{7}{c}{\textbf{Initial Solver Generalization}}                                                                                                                  \\ \midrule
    \multicolumn{1}{c|}{}                         & \multicolumn{2}{c|}{Agent Num}                                  & \multicolumn{2}{c|}{Our-SVM}          & \multicolumn{2}{c|}{Our-NNS}          & \multicolumn{1}{c|}{}                         & \multicolumn{2}{c|}{Initial Solution}                       & \multicolumn{2}{c|}{Our-SVM}          & \multicolumn{2}{c}{Our-NNS} \\ \midrule
    \multicolumn{1}{c|}{Map}                      & \multicolumn{1}{c}{Train} & \multicolumn{1}{c|}{Infer} & Delay   & \multicolumn{1}{c|}{AUC}    & Delay   & \multicolumn{1}{c|}{AUC}    & \multicolumn{1}{c|}{Map}                      & Train          & \multicolumn{1}{c|}{Infer}    & Delay   & \multicolumn{1}{c|}{AUC}    & Delay         & AUC         \\ \midrule
    \multicolumn{1}{c|}{random}  & \multicolumn{1}{c|}{250}   & \multicolumn{1}{c|}{350}   & 4800.2  & \multicolumn{1}{c|}{175.8}  & 5466.7  & \multicolumn{1}{c|}{193.5}  & \multicolumn{1}{c|}{random}  &    \multicolumn{1}{c|}{LNS2}        & \multicolumn{1}{c|}{LaCAM2}   & 1521.2  & \multicolumn{1}{c|}{67.43}  & 1747.1        & 70.88       \\
    \multicolumn{1}{c|}{+250/350}                         & \multicolumn{1}{c|}{350}   & \multicolumn{1}{c|}{350}   & 4806.75 & \multicolumn{1}{c|}{177.72} & 5513.13 & \multicolumn{1}{c|}{188.85} & \multicolumn{1}{c|}{+250}                         &    \multicolumn{1}{c|}{LaCAM2}         & \multicolumn{1}{c|}{LaCAM2}   & 1517.49 & \multicolumn{1}{c|}{61.41}  & 1811.4        & 65.67       \\\midrule
    \multicolumn{1}{c|}{random}                         & \multicolumn{1}{c|}{250}   & \multicolumn{1}{c|}{250}   & 1713.9  & \multicolumn{1}{c|}{59.1}   & 1683.7  & \multicolumn{1}{c|}{57.5}   & \multicolumn{1}{c|}{random}                         &        \multicolumn{1}{c|}{LNS2}       & \multicolumn{1}{c|}{EECBS}    & 1443.57 & \multicolumn{1}{c|}{49.98}  & 1604.85       & 53.9        \\
    \multicolumn{1}{c|}{+250/350}                         & \multicolumn{1}{c|}{350}   & \multicolumn{1}{c|}{250}   & 1578.61 & \multicolumn{1}{c|}{56.29}  & 1738.46 & \multicolumn{1}{c|}{60.36}  & \multicolumn{1}{c|}{+250}                         &      \multicolumn{1}{c|}{EECBS}        & \multicolumn{1}{c|}{EECBS}    & 1452.18 & \multicolumn{1}{c|}{51.38}  & 1591.58       & 53.67       \\ \midrule
    \multicolumn{1}{c|}{den520d} & \multicolumn{1}{c|}{700}   & \multicolumn{1}{c|}{900}   & 1816.6  & \multicolumn{1}{c|}{216.5}  & 1821.4  & \multicolumn{1}{c|}{168.1}  & \multicolumn{1}{c|}{den520d} &   \multicolumn{1}{c|}{LNS2}          & \multicolumn{1}{c|}{LaCAM2}   & 660.7   & \multicolumn{1}{c|}{327.11} & 816.6         & 726.01      \\ 
    \multicolumn{1}{c|}{+700/900}                         & \multicolumn{1}{c|}{900}   & \multicolumn{1}{c|}{900}   & 4171.37 & \multicolumn{1}{c|}{329.74} & 1426.54 & \multicolumn{1}{c|}{87.56}  & \multicolumn{1}{c|}{+700}                         &  \multicolumn{1}{c|}{LaCAM2}         & \multicolumn{1}{c|}{LaCAM2}   & 710.94  & \multicolumn{1}{c|}{127.99} & 771.46        & 79.05       \\  \midrule %\cmidrule(l){8-14} 
    \multicolumn{1}{c|}{den520d}                         & \multicolumn{1}{c|}{900}   & \multicolumn{1}{c|}{700}   & 931.5   & \multicolumn{1}{c|}{134.93} & 793.62  & \multicolumn{1}{c|}{67.29}  & \multicolumn{1}{c|}{Paris}   &   \multicolumn{1}{c|}{LNS2}         & \multicolumn{1}{c|}{EECBS}    & 113.36  & \multicolumn{1}{c|}{3.6}    & 125.22        & 4.06        \\
    \multicolumn{1}{c|}{+700/900}                         & \multicolumn{1}{c|}{700}   & \multicolumn{1}{c|}{700}   & 665.2   & \multicolumn{1}{c|}{77.9}   & 814     & \multicolumn{1}{c|}{68.2}   & \multicolumn{1}{c|}{+450}                         &     \multicolumn{1}{c|}{EECBS}       & \multicolumn{1}{c|}{EECBS}    & 115.68  & \multicolumn{1}{c|}{3.59}   & 131.88        & 4.2         \\ \bottomrule
    \end{tabular}
    }
    \end{table}




==> sup_table/svm_comp.tex <==
\begin{table}[h]
\caption{Average ranking of trained Orig-SVM-LNS and reported values by~\citet{huang2022anytime}. 'n' represents the number of agents in the map. }
  \label{table:svm-avg-rank}
  \centering
  {\small
  \begin{tabular}{c|c|c|c}
    \toprule
         % \multicolumn{4}{c}{Initial delays} \\ \midrule
        Map &  n & Our & Reported                             \\
    \midrule
    % empty & 300 & 12.08/20 & - \\
    % random-32-32-20 & 150 & 13.91/20  & - \\
    % random-32-32-10 & 100 & - & 6.5/20 \\
    warehouse & 100 & 5.89/20 & 6.0/20 \\
    ostd003d & 100 & 6.2/20 & 5.4/20 \\
    den520d  & 200 & 7.59/20 & 7.0/20 \\
    Paris & 250 & 7.75/20 & 6.7/20 \\
  \bottomrule
  \end{tabular}
  }
\end{table}


==> sup_table/test_table.tex <==


\begin{table}[h]
    \caption{Total iterations, final delays, and AUC in different evaluation cases within a time limit of \textbf{60s} and \textbf{300s}, using PP and PBS as replan solvers. The neighborhood selection strategy is RandomWalk with a neighborhood size of 25. 'In' refers to the algorithm used for finding initial solutions. For both final delays and AUC, lower values are better. The settings where PBS performs better are highlighted in red, for all other settings, PP is superior.}
    \label{table:pp-pbs-60s}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}|c|c|c|cc|cc|cc|c|c|c|cc|cc|cc|@{}}
    \toprule
    \multicolumn{18}{|c|}{\textbf{Run Time Limit: 60s}} \\ 
    \midrule
    \multirow{3}{*}{} & \multirow{3}{*}{In} & \multirow{3}{*}{n} & \multicolumn{2}{c|}{Iter (x1k)} & \multicolumn{2}{c|}{Final delays} & \multicolumn{2}{c|}{AUC (x10k)} & \multirow{3}{*}{} & \multirow{3}{*}{In} & \multirow{3}{*}{n} & \multicolumn{2}{c|}{Iter (x1k)} & \multicolumn{2}{c|}{Final delays} & \multicolumn{2}{c|}{AUC (x10k)} \\
    \cmidrule(lr){4-9} \cmidrule(lr){13-18}
    & & & PP & PBS & PP & PBS & PP & PBS & & & & PP & PBS & PP & PBS & PP & PBS \\
    \midrule
    \multirow{10}{*}{\rotatebox{90}{empty}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 300 & 8.21 & 0.48 & 439.6 & \textcolor{red}{424.5} & 3.89 & 6.07 & \multirow{10}{*}{\rotatebox{90}{random}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 150 & 6.21 & 0.58 & 352.1 & \textcolor{red}{343.1} & 2.5 & 3.6 \\
     &  & 350 & 4.13 & 0.22 & 1,127.6 & 1,286.8 & 9.4 & 14.2 &  &  & 200 & 3.01 & 0.20 & 952.5 & \textcolor{red}{874.9} & 7.3 & 7.6 \\
     &  & 400 & 2.24 & 0.12 & 2,663.1 & 2,982.4 & 20.2 & 27.1 &  &  & 250 & 2.22 & 0.07 & 2,449.5 & \textcolor{red}{2,443.6} & 18.6 & 21.7 \\
     &  & 450 & 2.15 & 0.11 & 5,110.7 & 5,211.0 & 36.9 & 41.4 &  &  & 300 & 2.03 & 0.04 & 5,318.2 & 5,693.2 & 39.6 & 44.9 \\
     &  & 500 & 2.40 & 0.08 & 8,400.6 & 8,815.3 & 59.2 & 64.5 &  &  & 350 & 2.61 & 0.00 & 14,729.1 & \textcolor{red}{14,630.2} & 82.4 & 83.7 \\
    \cmidrule(lr){2-9} \cmidrule(lr){11-18}
    & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 300 & 8.98 & 0.44 & 431.7 & 436.9 & 3.5 & 4.8 & & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 150 & 7.39 & 0.63 & 350.1 & \textcolor{red}{346.9} & 2.3 & 2.8 \\
     &  & 350 & 4.22 & 0.25 & 1,109.8 & \textcolor{red}{1,081.8} & 8.7 & 9.8 &  &  & 200 & 2.88 & 0.19 & 959.6 & \textcolor{red}{875.5} & 6.8 & \textcolor{red}{6.5} \\
     &  & 400 & 2.28 & 0.15 & 2,570.1 & \textcolor{red}{2,238.2} & 18.7 & \textcolor{red}{17.5} &  &  & 250 & 1.99 & 0.05 & 2,423.8 & \textcolor{red}{2,301.4} & 16.7 & \textcolor{red}{16.2} \\
     &  & 450 & 1.83 & 0.09 & 4,873.5 & \textcolor{red}{4,293.6} & 32.7 & \textcolor{red}{29.9} &  &  & 300 & 1.47 & 0.03 & 5,309.6 & \textcolor{red}{4,533.1} & 33.7 & \textcolor{red}{30.4} \\
     &  & 500 & 1.51 & 0.05 & 7,817.6 & \textcolor{red}{6,874.2} & 49.3 & \textcolor{red}{45.2} &  &  & 350 & 1.57 & 0.02 & 8,966.9 & \textcolor{red}{8,076.5} & 54.7 & \textcolor{red}{51.2} \\
    \midrule
    \multirow{10}{*}{\rotatebox{90}{warehouse}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 150 & 6.41 & 0.60 & 116.8 & 133.1 & 1.4 & 6.6 & \multirow{10}{*}{\rotatebox{90}{ost003d}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 200 & 1.73 & 0.09 & 198.5 & 1,074.5 & 3.7 & 12.4 \\
     &  & 200 & 2.94 & 0.25 & 259.8 & 319.3 & 7.3 & 7.6 &  &  & 300 & 0.93 & 0.07 & 988.8 & 3,117.1 & 13.9 & 35.6 \\
     &  & 250 & 1.74 & 0.13 & 486.7 & 941.4 & 18.6 & 21.7 &  &  & 400 & 0.57 & 0.03 & 3,285.9 & 9,320.1 & 37.3 & 81.6 \\
     &  & 300 & 1.06 & 0.07 & 845.2 & 2,987.7 & 39.6 & 44.9 &  &  & 500 & 0.19 & 0.01 & 12,164.9 & 21,539.9 & 98.6 & 145.5 \\
     &  & 350 & 0.65 & 0.03 & 1,625.8 & 7,963.7 & 82.4 & 83.7 &  &  & 600 & 0.13 & 0.01 & 27,290.3 & 35,498.7 & 188.7 & 221.2 \\
    \cmidrule(lr){2-9} \cmidrule(lr){11-18}
    & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 150 & 6.59 & 0.57 & 122.1 & 128.3 & 2.3 & 2.8 & & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 200 & 1.75 & 0.06 & 183.9 & 897.6 & 2.8 & 9.5 \\
     &  & 200 & 2.65 & 0.27 & 266.8 & 310.2 & 6.8 & \textcolor{red}{6.5} &  &  & 300 & 0.92 & 0.02 & 915.5 & 4,630.9 & 12.3 & 35.2 \\
        &  & 250 & 1.83 & 0.15 & 477.6 & 760.3 & 16.7 & \textcolor{red}{16.2} &  &  & 400 & 0.52 & 0.03 & 3,230.7 & 8,032.7 & 32.4 & 62.3 \\
        &  & 300 & 1.15 & 0.09 & 832.7 & 1,740.3 & 33.7 & \textcolor{red}{30.4} &  &  & 500 & 0.21 & 0.01 & 9,335.3 & 16,709.3 & 72.3 & 107.8 \\
        &  & 350 & 0.73 & 0.06 & 1,495.0 & 3,237.5 & 54.7 & \textcolor{red}{51.2} &  &  & 600 & 0.15 & 0.01 & 17,998.3 & 24,525.7 & 125.2 & 152.2 \\
    \midrule
    \multirow{10}{*}{\rotatebox{90}{den520d}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 500 & 1.44 & 0.04 & 871.6 & 8,082.4 & 18.5 & 77.1 & \multirow{10}{*}{\rotatebox{90}{Paris}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 350 & 7.48 & 0.16 & 99.8 & 817.8 & 1.8 & 18.5 \\
     &  & 600 & 1.07 & 0.02 & 2,266.5 & 17,753.3 & 35.3 & 129.3 &  &  & 450 & 6.69 & 0.10 & 134.3 & 3,032.1 & 6.2 & 79.9 \\
     &  & 700 & 0.86 & 0.02 & 4,396.1 & 24,979.7 & 57.9 & 175.6 &  &  & 550 & 5.37 & 0.05 & 213.7 & 8,664.9 & 10.6 & 119.2 \\
     &  & 800 & 0.53 & 0.01 & 9,205.8 & 35,921.6 & 96.9 & 234.4 &  &  & 650 & 4.58 & 0.03 & 298.0 & 15,771.8 & 18.5 & 165.3 \\
     &  & 900 & 0.49 & 0.01 & 12,900.4 & 45,686.7 & 124.4 & 291.1 &  &  & 750 & 3.57 & 0.02 & 483.6 & 24,171.6 & 18.5 & 165.3 \\
    \cmidrule(lr){2-9} \cmidrule(lr){11-18}
    & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 500 & 1.28 & 0.05 & 899.6 & 6,195.8 & 15.9 & 52.9 & & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 350 & 5.98 & 0.17 & 82.2 & 383.7 & 1.0 & 8.4 \\
     &  & 600 & 1.72 & 0.06 & 1,321.3 & 8,485.5 & 29.8 & 79.2 &  &  & 450 & 6.44 & 0.11 & 138.7 & 2,274.2 & 1.8 & 22.8 \\
     &  & 700 & 0.78 & 0.02 & 4,436.5 & 16,642.9 & 49.1 & 111.9 &  &  & 550 & 4.72 & 0.06 & 219.3 & 4,878.6 & 4.1 & 46.0 \\
     &  & 800 & 0.61 & 0.02 & 7,342.8 & 21,909.0 & 73.2 & 142.2 &  &  & 650 & 4.49 & 0.04 & 317.1 & 9,304.6 & 4.6 & 14.7 \\
     &  & 900 & 0.44 & 0.01 & 13,032.0 & 29,352.2 & 105.6 & 181.4 &  &  & 750 & 3.07 & 0.03 & 614.9 & 14,707.1 & 14.8 & 104.5 \\
    \bottomrule
    \end{tabular}
    }

 
    
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}|c|c|c|cc|cc|cc|c|c|c|cc|cc|cc|@{}}
    \toprule
    \multicolumn{18}{|c|}{\textbf{Run Time Limit: 300s}} \\ 
    \midrule
    \multirow{3}{*}{} & \multirow{3}{*}{In} & \multirow{3}{*}{n} & \multicolumn{2}{c|}{Iter (x10k)} & \multicolumn{2}{c|}{Final delays} & \multicolumn{2}{c|}{AUC (x10k)} & \multirow{3}{*}{} & \multirow{3}{*}{In} & \multirow{3}{*}{n} & \multicolumn{2}{c|}{Iter (x10k)} & \multicolumn{2}{c|}{Final delays} & \multicolumn{2}{c|}{AUC (x10k)} \\
    \cmidrule(lr){4-9} \cmidrule(lr){13-18}
    & & & PP & PBS & PP & PBS & PP & PBS & & & & PP & PBS & PP & PBS & PP & PBS \\
    \midrule
    \multirow{10}{*}{\rotatebox{90}{empty}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 300 & 4.29 & 0.21 & 367.93 & \textcolor{red}{332.33} & 13.31 & 14.58 & \multirow{10}{*}{\rotatebox{90}{random}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 150 & 3.11 & 0.24 & 329.46 & \textcolor{red}{321.35} & 10.62 & 11.40 \\
     &  & 350 & 2.07 & 0.12 & 840.33 & \textcolor{red}{692.63} & 31.70 & 33.88 &  &  & 200 & 1.58 & 0.10 & 789.77 & \textcolor{red}{723.64} & 27.32 & \textcolor{red}{25.79} \\
     &  & 400 & 1.09 & 0.06 & 1971.57 & \textcolor{red}{1544.34} & 73.21 & 75.04 &  &  & 250 & 1.24 & 0.03 & 1857.06 & \textcolor{red}{1618.02} & 67.80 & \textcolor{red}{66.54} \\
     &  & 450 & 1.07 & 0.04 & 3899.78 & \textcolor{red}{3258.99} & 140.35 & 135.04 &  &  & 300 & 1.21 & 0.02 & 4102.65 & \textcolor{red}{3602.96} & 147.89 & \textcolor{red}{145.24} \\
     &  & 500 & 1.28 & 0.03 & 6615.22 & \textcolor{red}{6092.54} & 232.28 & \textcolor{red}{231.80} &  &  & 350 & 1.06 & 0.01 & 8553.05 & \textcolor{red}{7610.30} & 315.27 & \textcolor{red}{310.00} \\
    \cmidrule(lr){2-9} \cmidrule(lr){11-18}
    & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 300 & 4.64 & 0.19 & 363.99 & \textcolor{red}{338.95} & 12.64 & 13.45 & & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 150 & 3.78 & 0.23 & 333.89 & \textcolor{red}{328.94} & 10.48 & 10.81 \\
     &  & 350 & 2.09 & 0.12 & 853.13 & \textcolor{red}{695.69} & 31.16 & \textcolor{red}{28.84} &  &  & 200 & 1.53 & 0.10 & 812.82 & \textcolor{red}{741.66} & 27.44 & 25.24 \\
     &  & 400 & 1.10 & 0.07 & 1920.56 & \textcolor{red}{1400.21} & 69.98 & \textcolor{red}{57.49} &  &  & 250 & 1.21 & 0.03 & 1841.19 & \textcolor{red}{1651.25} & 65.43 & 61.16 \\
     &  & 450 & 1.00 & 0.04 & 3749.88 & \textcolor{red}{3010.31} & 132.28 & \textcolor{red}{112.73} &  &  & 300 & 0.95 & 0.01 & 4253.84 & \textcolor{red}{3527.62} & 146.07 & 123.06 \\
     &  & 500 & 0.98 & 0.02 & 6447.52 & \textcolor{red}{5352.49} & 216.74 & \textcolor{red}{186.70} &  &  & 350 & 0.87 & 0.01 & 8225.15 & \textcolor{red}{6477.20} & 260.50 & \textcolor{red}{221.69} \\
    \midrule
    \multirow{10}{*}{\rotatebox{90}{warehouse}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 150 & 3.01 & 0.19 & 113.44 & 126.99 & 4.14 & 9.70 & \multirow{10}{*}{\rotatebox{90}{ost003d}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 200 & 0.87 & 0.04 & 154.04 & 278.75 & 7.60 & 24.60 \\
     &  & 200 & 1.48 & 0.12 & 247.88 & 262.47 & 9.40 & 16.07 &  &  & 300 & 0.50 & 0.03 & 381.95 & 1160.64 & 26.76 & 82.84 \\
     &  & 250 & 0.93 & 0.08 & 435.51 & 445.94 & 18.17 & 38.03 &  &  & 400 & 0.37 & 0.02 & 1009.37 & 4071.87 & 76.53 & 207.71 \\
     &  & 300 & 0.55 & 0.05 & 678.67 & 741.87 & 31.86 & 74.78 &  &  & 500 & 0.13 & 0.01 & 4618.86 & 9758.70 & 275.91 & 483.51 \\
     &  & 350 & 0.35 & 0.03 & 1082.86 & 1471.08 & 61.14 & 154.76 &  &  & 600 & 0.07 & 0.00 & 15629.46 & 26768.67 & 691.40 & 960.09 \\
    \cmidrule(lr){2-9} \cmidrule(lr){11-18}
    & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 150 & 2.11 & 0.19 & 117.88 & 123.87 & 3.74 & 6.44 & & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 200 & 0.50 & 0.02 & 152.40 & 273.43 & 6.69 & 19.75 \\
     &  & 200 & 0.98 & 0.11 & 247.48 & 261.31 & 8.25 & 11.05 &  &  & 300 & 0.40 & 0.01 & 384.24 & 1976.41 & 24.38 & 106.45 \\
     &  & 250 & 0.70 & 0.07 & 431.72 & 462.32 & 15.25 & 21.93 &  &  & 400 & 0.31 & 0.01 & 1047.86 & 4422.10 & 72.15 & 192.26 \\
        &  & 300 & 0.55 & 0.05 & 694.66 & 757.45 & 26.39 & 41.51 &  &  & 500 & 0.15 & 0.01 & 3671.84 & 10219.26 & 204.61 & 417.48 \\
        &  & 350 & 0.36 & 0.03 & 1042.26 & 1365.12 & 43.40 & 75.23 &  &  & 600 & 0.08 & 0.00 & 11333.95 & 19107.23 & 465.10 & 668.65 \\
    \midrule 
    \multirow{10}{*}{\rotatebox{90}{den520d}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 500 & 7.41 & 0.24 & 313.61 & 2545.75 & 28.71 & 174.77 & \multirow{10}{*}{\rotatebox{90}{Paris}} & \multirow{5}{*}{\rotatebox{90}{LaCAM2}} & 350 & 35.13 & 0.70 & 99.32 & \textcolor{red}{98.29} & 4.23 & 22.87 \\
     &  & 600 & 5.34 & 0.14 & 612.69 & 5572.76 & 59.27 & 355.08 &  &  & 450 & 31.77 & 0.48 & 130.44 & 273.60 & 6.32 & 65.28 \\
     &  & 700 & 4.52 & 0.12 & 1110.30 & 8460.08 & 104.28 & 525.67 &  &  & 550 & 25.61 & 0.33 & 203.97 & 1520.53 & 11.17 & 168.08 \\
     &  & 800 & 2.79 & 0.08 & 2410.77 & 16784.33 & 198.78 & 832.76 &  &  & 650 & 22.87 & 0.21 & 267.48 & 4650.54 & 17.19 & 302.78 \\
     &  & 900 & 2.75 & 0.06 & 3648.21 & 27560.22 & 274.32 & 1148.42 &  &  & 750 & 16.96 & 0.15 & 366.11 & 8294.67 & 27.73 & 506.11 \\
    \cmidrule(lr){2-9} \cmidrule(lr){11-18}
    & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 500 & 6.64 & 0.24 & 296.55 & 2551.81 & 26.00 & 146.33 & & \multirow{5}{*}{\rotatebox{90}{LNS2}} & 350 & 20.20 & 0.71 & 80.40 & 100.92 & 2.96 & 11.59 \\
     &  & 600 & 5.23 & 0.16 & 583.83 & 5301.91 & 52.54 & 241.87 &  &  & 450 & 24.70 & 0.50 & 136.48 & 216.70 & 5.15 & 38.58 \\
     &  & 700 & 4.07 & 0.12 & 1196.94 & 8145.64 & 97.44 & 384.84 &  &  & 550 & 12.81 & 0.33 & 205.32 & 1159.81 & 9.14 & 107.83 \\
     &  & 800 & 3.27 & 0.11 & 2076.04 & 12242.85 & 159.80 & 535.81 &  &  & 650 & 20.25 & 0.23 & 280.04 & 3657.95 & 14.13 & 203.35 \\
     &  & 900 & 2.33 & 0.03 & 3979.49 & 23163.43 & 262.41 & 807.24 &  &  & 750 & 9.60 & 0.17 & 414.18 & 6561.66 & 25.51 & 323.93 \\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> table/nns_comp.tex <==

\begin{table}[t]
\caption{Delay elimination after 100 iterations of our trained Neural-LNS versus its reported performance in shared maps, by starting from roughly the same initial delays.}

\vspace{-6pt}
\label{table:neural-100iter}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}cc|cc|cc|cc@{}}
\toprule
                               &     & \multicolumn{2}{c|}{Initial delays} & \multicolumn{2}{c|}{Starting Iteration} & \multicolumn{2}{c}{Delay elimination} \\ \midrule
\multicolumn{1}{c|}{Map}       & N   & Our              & Reported         & Our              & Reported             & Our              & Reported         \\ \midrule
\multicolumn{1}{c|}{empty}     & 300 & 3140.7           & 3200             & 0                & 0                    & 2202             & 1850             \\
\multicolumn{1}{c|}{warehouse} & 100 & 5731.8           & 5500             & 2                & 0                    & 4908             & 4700             \\
\multicolumn{1}{c|}{ost003d}   & 100 & 8690.4           & 8600             & 39               & 0                    & 4585.1           & 5000             \\
\multicolumn{1}{c|}{den520d}   & 200 & 20510.2          & 20500            & 19               & 0                    & 12721.3          & 14500            \\ \bottomrule
\end{tabular}
}


\vspace{4pt} % Ensure the space is noticeable, increase if needed
\parbox{0.45\textwidth}{\scriptsize Note: 'N' is the number of agents. 'Our' refers to our recovered results. 'Reported' refers to values given by \citet{yan2024neural}. 
}

\vspace{-8pt}

\end{table}

%  of trained Ori-Neural-LNS within 100 iterations and reported values by \cite{yan2024neural},  if starting from a roughly equivalent point of delays. 'n' represent the number of agents in the map.
